RAVEN: Rethinking Adversarial Video Generation with Efficient Tri-plane Networks

We present a novel unconditional video generative model designed to address long-term spatial and temporal dependencies, with attention to computational and dataset efficiency. To capture long spatio-temporal dependencies, our approach incorporates a hybrid explicit-implicit tri-plane representation inspired by 3D-aware generative frameworks developed for three-dimensional object representation and employs a single latent code to model an entire video clip. Individual video frames are then synthesized from an intermediate tri-plane representation, which itself is derived from the primary latent code. This novel strategy more than halves the computational complexity measured in FLOPs compared to the most efficient state-of-the-art methods. Consequently, our approach facilitates the efficient and temporally coherent generation of videos. Moreover, our joint frame modeling approach, in contrast to autoregressive methods, mitigates the generation of visual artifacts. We further enhance the model's capabilities by integrating an optical flow-based module within our Generative Adversarial Network (GAN) based generator architecture, thereby compensating for the constraints imposed by a smaller generator size. As a result, our model synthesizes high-fidelity video clips at a resolution of $256\times256$ pixels, with durations extending to more than $5$ seconds at a frame rate of 30 fps. The efficacy and versatility of our approach are empirically validated through qualitative and quantitative assessments across three different datasets comprising both synthetic and real video clips. We will make our training and inference code public.

==> sec/sup_mat.tex <==
\clearpage
\setcounter{page}{1}
\maketitlesupplementary

\section{Real Data} Along with this PDF in our supplementary material, you will find a .zip archive that holds sample videos from our training dataset. Note that we face similar problems finding suitable data as noted in~\cite{brooks2022generating,skorokhodov2022stylegan}. The problems namely are — modern datasets of videos are either too small (only a few 100s videos (Fashion videos, FaceForensics, CelebV-HQ)), too simple ((Synthetically generated videos of NeRF objects)No object articulation, only camera motion, etc.), or too complex (very wide collection of videos of random scenes (Kinetics-600, UCF-101)). Therefore, we use clever `animation' techniques to increase data volume, as described in~\cref{subsec:datasets}. However, the methods we use are not perfect and produce artifacts depending upon the source-appearance and motion. Furthermore, we found with a manual inspection that these methods~\cite{zhao2022thin,yu2023bidirectionally}, although state-of-the-art, have the effect of generating videos with limited motion. This is then carried over to the final result of our method. Therefore, for manual judgment of generation quality, we highly recommend an inspection of the training data. In the directory named real\_samples, there are $3$ subdirectories, each containing $32$ random sample videos corresponding to each dataset.

\section{Generated data} In the directory named generated\_samples, there are $5$ subdirectories corresponding to each of the models we train. Each of these subdirectories in tern contains $3$ directories corresponding to each dataset, and each of them contains $32$ random sample videos.

\section{Extrapolation with triplane representation}
\begin{table*}[h!]
\centering
    \begin{tabular}{lcccccccccccc}
        \toprule
        & \multicolumn{4}{c}{Talking Faces all Motions} & \multicolumn{4}{c}{Fashion Videos} & \multicolumn{4}{c}{UCF 101} \\
        \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
        Method     & \multicolumn{2}{c}{3 frame interp.} & \multicolumn{2}{c}{8 frame intrp.}& \multicolumn{2}{c}{3 frame interp.} & \multicolumn{2}{c}{8 frame intrp.}& \multicolumn{2}{c}{3 frame interp.} & \multicolumn{2}{c}{8 frame intrp.} \\ 
        \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}\cmidrule(lr){12-13}
         & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR \\
        \midrule
        Pos. emb & 0.17 &15.26 &0.17 &15.19 &0.70 &17.41 &0.70 &17.59 &0.17 &14.29 &0.21 &14.39  \\
        voxels & 0.73 &25.71 &0.71 &24.77 &0.86 &24.87 &0.85 &23.95 &0.46 &19.54 &0.46 &19.57  \\
        triplane  & 0.83 &28.49 &0.82 &27.61 &0.91 &27.65 &\textbf{0.90} &26.40 &0.50 &19.87 &0.50 &19.88  \\
        triplane+flow & \textbf{0.86} &\textbf{29.76} &\textbf{0.84} &\textbf{28.32} &\textbf{0.92} &\textbf{28.25} &\textbf{0.90} &\textbf{26.65} &\textbf{0.51} &\textbf{20.25} &\textbf{0.52} &\textbf{20.11}  \\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Tri-plane video representation for extrapolation:} We compare the effectiveness of the tri-plane representation for Video data by computing SSIM and PSNR value of extrapolated frames. Note that for all metric, higher is better. The reported numbers here are average PSNR over $20$ random videos taken from each of our data sets}
    \label{table:quantitative_comaprison_extrapolation}
\end{table*}

